AMSbench: A Comprehensive Benchmark for Evaluating MLLM Capabilities in AMS Circuits

Analog/Mixed-Signal (AMS) circuits play a critical role in the integrated circuit (IC) industry. However, automating Analog/Mixed-Signal (AMS) circuit design has remained a longstanding challenge due to its difficulty and complexity. Although recent advances in Multi-modal Large Language Models (MLLMs) offer promising potential for supporting AMS circuit analysis and design, current research typically evaluates MLLMs on isolated tasks within the domain, lacking a comprehensive benchmark that systematically assesses model capabilities across diverse AMS-related challenges. To address this gap, we introduce AMSbench, a benchmark suite designed to evaluate MLLM performance across critical tasks including circuit schematic perception, circuit analysis, and circuit design. AMSbench comprises approximately 8000 test questions spanning multiple difficulty levels and assesses eight prominent models, encompassing both open-source and proprietary solutions such as Qwen 2.5-VL and Gemini 2.5 Pro. Our evaluation highlights significant limitations in current MLLMs, particularly in complex multi-modal reasoning and sophisticated circuit design tasks. These results underscore the necessity of advancing MLLMs' understanding and effective application of circuit-specific knowledge, thereby narrowing the existing performance gap relative to human expertise and moving toward fully automated AMS circuit design workflows. Our data is released at this URL.

==> tables/Design_Testbench.tex <==
% 定义新的列类型 L，用于左对齐数据，标题居中
\newcolumntype{L}{>{\raggedright\arraybackslash}X}

\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{P}{>{\centering\arraybackslash}p{2cm}}
\newcolumntype{E}{>{\centering\arraybackslash}X}
\begin{table}[ht]
\tiny % 减小字体大小以避免文字挤压
\centering
\begin{tabularx}{\textwidth}{@{}l *{4}{C} p{0.3cm} *{5}{C}@{}}
% \begin{tabular}{@{}lccccccc|cc|c@{}}
\toprule
\textbf{MODEL} & \multicolumn{7}{c}{\textbf{OTA}} & \multicolumn{2}{c}{\textbf{Comparator}} & \multicolumn{1}{c}{\textbf{Bootstrap}} \\
\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
 & \textbf{CMRR} & \textbf{DC gain} & \textbf{GBW} & \textbf{Phase margin} & \textbf{Power} & \textbf{PSR} & \textbf{SR} & \textbf{Delay} & \textbf{Offset} & \textbf{ENOB} \\
\midrule
Gemini2.5 pro & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
gpt4o & 0 (1) & 0 & 0 & 0 & \textbf{0(1,2,3,5)} & \textbf{0(1,2)} & 0 & \textbf{0(1,2)} & \textbf{0(2,4)} & 0 \\
Claude3.7 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Grok3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
doubao & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
KIMI-VL-A3B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Qwen2.5-VL-72B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabularx}

\caption{OTA, Comparator, and Bootstrap Performance Across Different Models}
\label{tab:ota_comparator_performance}
\end{table}


\begin{table}[ht]
\tiny % 减小字体大小以避免文字挤压
\centering
\begin{tabularx}{\textwidth}{@{}l *{4}{C} p{0.3cm} *{5}{C}@{}}
\toprule
\textbf{MODEL} & \multicolumn{7}{c}{\textbf{Telescope Amplifier}} & \multicolumn{2}{c}{\textbf{PLL}} & \multicolumn{1}{c}{\textbf{MOS}} \\
\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
 & \textbf{CMRR} & \textbf{DC gain} & \textbf{GBW} & \textbf{Phase margin} & \textbf{Power} & \textbf{PSR} & \textbf{SR} & \textbf{Jitter} & \textbf{Phase noise} & \textbf{Ron} \\
\midrule
Gemini2.5 pro & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
gpt4o & 0  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Claude3.7 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Grok3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
doubao & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
KIMI-VL-A3B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Qwen2.5-VL-72B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabularx}
\caption{Telescope Amplifier, PLL, and MOS Performance Across Different Models}
\label{tab:ota_comparator_performance}
\end{table}


\begin{table}[ht]
\tiny % 减小字体大小以避免文字挤压
\centering
\begin{tabularx}{\textwidth}{@{}l *{4}{C} p{0.75cm} *{5}{C}@{}}
\toprule
\textbf{MODEL} & \multicolumn{7}{c}{\textbf{LDO}} & \multicolumn{2}{c}{\textbf{PLL-VCO}} & \multicolumn{1}{c}{\textbf{Unit cap}} \\
\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
 & \textbf{LDR} & \textbf{LNR} & \textbf{Drop voltage} & \textbf{DC gain} & \textbf{Phase margin} & \textbf{PSR} & \textbf{Offset} & \textbf{Jitter} & \textbf{Phase noise} & \textbf{MC-mismatch} \\
\midrule
Gemini2.5 pro & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
gpt4o & 0  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \textbf{0(1,2,3)} \\
Claude3.7 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Grok3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
doubao & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
KIMI-VL-A3B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Qwen2.5-VL-72B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabularx}
\caption{LDO, PLL-VCO, and Unit\_cap Performance Across Different Models}
\label{tab:ota_comparator_performance}
\end{table}

\begin{table}[ht]
\tiny % 减小字体大小以避免文字挤压
\centering
\begin{tabularx}{\textwidth}{@{}l *{4}{C} p{0.75cm} *{5}{C}@{}}
\toprule
\textbf{MODEL} & \multicolumn{5}{c}{\textbf{Folded Amplifier}} & \multicolumn{1}{c}{\textbf{SAR ADC}} & \multicolumn{4}{c}{\textbf{Bandgap}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-7} \cmidrule(lr){8-11}
 & \textbf{DC gain} & \textbf{SR} & \textbf{Phase margin} & \textbf{GBW} & \textbf{Power} & \textbf{ENOB} & \textbf{BuildiupV} & \textbf{Noise} & \textbf{PSR} & \textbf{TC} \\
\midrule
Gemini2.5 pro & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
gpt4o & 0  & 0 & 0 & 0 & 0 & 0 & 0 & \textbf{0(3)} & 0 & 0 \\
Claude3.7 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Grok3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
doubao & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
KIMI-VL-A3B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
Qwen2.5-VL-72B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabularx}
\caption{Fold-amp, SAR ADC, and Bandgap Performance Across Different Models}
\label{tab:ota_comparator_performance}
\end{table}
